A Non-Intrusive Correction Algorithm for Classification Problems with Corrupted Data

A novel correction algorithm is proposed for multi-class classification problems with corrupted training data. The algorithm is non-intrusive, in the sense that it post-processes a trained classification model by adding a correction procedure to the model prediction. The correction procedure can be coupled with any approximators, such as logistic regression, neural networks of various architectures, etc. When training dataset is sufficiently large, we prove that the corrected models deliver correct classification results as if there is no corruption in the training data. For datasets of finite size, the corrected models produce significantly better recovery results, compared to the models without the correction algorithm. All of the theoretical findings in the paper are verified by our numerical examples.

==> FirstVersion(arxiv)/Analysis.tex <==
\section{Main Theoretical Analysis} \label{sec:analysis}
%In this section, we present our theoretical analysis and algorithm.

%\subsection{Theoretical Analysis}

In this subsection, we present theoretical analysis for the above
classification problem. We first derive conditions on the corruption
ratio $\lambda$ and the distribution $\{\alpha_k\}_{1\leq k\leq n}$,
under which the CCE and the SE loss functions are inherently robust
against the label corruption.  Based upon the analysis, we propose a
modified classifier, to be used after data training, to
eliminate the impact of corrupted data. 

\subsection{Asymptotic Empirical Risk}
%Note that it is rather difficult to analyze the minimum of ${\mathcal E} ({\bf q})$, which is data-dependent. 
Most of analysis is based on the assumption that the data set $S$ is sufficiently large, i.e., $M\gg 1$. 
%
Let $S_j := (S\setminus S_c) \cap D_j$, $j=1,\dots, n$. 
The empirical risk \eqref{risk} can be split into $n+1$ parts as 
\begin{equation*}
\begin{aligned}
{\mathcal E}( \f ) &= \sum_{j=1}^n \bigg(  \frac{1}{M}  \sum_{ \x_i \in S_j  } L ( \ty ( \x_i), \f ( \x_i) )  \bigg)
+ \frac{1}{M} 
\sum_{ \x_i \in S_c  } L ( \ty ( \x_i), \f ( \x_i) )
\\
&= \sum_{j=1}^n \bigg(  \frac{1}{M}  \sum_{ \x_i \in S_j  }  L ( {\bf e}_j, \f ( \x_i) )  \bigg)
+\frac{1}{M} 
\sum_{ \x_i \in S_c  } L ( \ty ( \x_i), \f ( \x_i) )
\\  
& =: \sum_{j=1}^n {\mathcal E}_j  + {\mathcal E}_c.
\end{aligned}
\end{equation*}

When$M \gg 1$, the following approximation holds: 
\begin{align}\label{app1}
\begin{aligned}
{\mathcal E}_j 
& \approx   (1-\lambda) \int_{D_j}   L ( {\bf e}_j, \f ( \x) )  d \omega_j, \quad 1\le j \le n,
\end{aligned}
\end{align}
where $d \omega_j =  \frac1{ \int_{D_j} d \omega } d \omega $.  
Note that for all $ \x_i \in S_c$, the label $ \ty ( \x_i)$ 
 is a realization of the random variable $\mathbf{Y}$ with the
 distribution \eqref{Yprob}. When $M \gg 1$, the summation in $
 {\mathcal E}_c$ can be considered as approximation to  expectation,
\begin{equation}\label{app2}
\begin{aligned}
{\mathcal E}_c \approx \lambda \sum_{j=1}^n  \int_{D_j} \bigg(  \sum_{k=1}^n \alpha_k 
L ( {\bf e}_k, \f ( \x ) )
\bigg) d \omega_j.
\end{aligned}
\end{equation}
Therefore, when $M \gg 1$, we have 
\begin{equation}
  \label{Jf}
\begin{split} 
{\mathcal E} (\f ) & \approx 
(1-\lambda) \sum_{j=1}^n \int_{D_j}  L ( {\bf e}_j, \f ( \x) )  d \omega_j
+ \lambda \sum_{j=1}^n  \int_{D_j} \bigg(  \sum_{k=1}^n \alpha_k 
L ( {\bf e}_k, \f ( \x) )
\bigg) d \omega_j
\\
& =  \sum_{j=1}^n \int_{D_j} \bigg( (1-\lambda) L ( {\bf e}_j, \f ( \x) )
+  \lambda  \sum_{k=1}^n \alpha_k 
L ( {\bf e}_k, \f (\x) )
\bigg ) d \omega_j
\\
& =: J( \f ).
\end{split}
\end{equation}


%The functional $J( \f )$ is an accurate approximation to  ${\mathcal E} (\f )$ when the amount of the data set $S$ is sufficiently large. 
As the number of data $M \rightarrow +\infty$, the empirical risk ${\mathcal E} (\f )$ approaches $J( \f )$. Subsequently, we call $J( \f )$ {\it asymptotic empirical risk}. 
%Compared to ${\mathcal E} (\f )$, analyzing the minimum of $J( \f )$ is much easier. 

\subsection{Main Results}
Our main theoretical results are summarized as follows.

\begin{theorem} \label{thm:nd}
	For both the CCE and SE loss functions \eqref{eq:cce_mse_loss}, 
	the function $\f^* $ that minimizes the asymptotic empirical
        risk $J(\f)$ \eqref{Jf} is 
	\begin{equation}\label{minf:n}
	\f^* ( \x ) = \begin{cases}
	\left( 1-\lambda + \lambda \alpha_1 , 
	\lambda \alpha_2,
	\dots, 
	\lambda \alpha_n
	\right), \quad &{\rm if}~\x\in D_1 ,
	\\
	\cdots &
	\\
	\left( \lambda \alpha_1 , \dots
\lambda \alpha_{j-1}, 1-\lambda + \lambda \alpha_j, \lambda \alpha_{j+1}
\dots, 
\lambda \alpha_n
\right), \quad &{\rm if}~\x\in D_j ,	1<j<n,
	\\
	\cdots &
	\\
	\left(  \lambda \alpha_1 , 
	\lambda \alpha_2,
	\dots, 
	1-\lambda + \lambda \alpha_n 
	\right), \quad &{\rm if}~\x\in D_n .		
	\end{cases}
	\end{equation}	
\end{theorem}

The proof of Theorem \ref{thm:nd} can be found in Appendix \ref{app1:proof}.

\begin{remark}
Theorem \ref{thm:nd} implies that the classification is completely recovered if and only if 
\begin{equation}
1-\lambda + \lambda \alpha_j > \lambda \max_{k \ne j} \{\alpha_k\}, \qquad j=1,\dots,n,
\end{equation}
or equivalently, 
%	\begin{equation}\label{ReCondition}
%	\lambda < \frac{1}{ 1+ \max_{j} \Big\{   \max_{k \neq j} \{\alpha_k\} - \alpha_j \Big\} }.
%	\end{equation}

\begin{equation}\label{ReCondition}
	\lambda < \frac{1}{ 1+ \max_{k} \{\alpha_k\}-\min_{k}\{\alpha_k\}}.
\end{equation}
In other words, under the condition \eqref{ReCondition}, it holds $\hf^* (\x) = \y( \x)$ for all $\x \in {\mathcal X}$.
\end{remark}

\begin{remark}
	Since $0\leq \alpha_k\leq 1$ for any $k$, a direct consequence of the condition \eqref{ReCondition} is that when $\lambda<\frac 12$, the classification can always be completely recoverred, given any corruption distribution $\{\alpha_k\}$.
\end{remark}

As a direct consequence of the above theorem, we have the following results for two special cases. 

\begin{corollary}\label{cor:2d}
Consider binary classification problem with  $n=2$ and corruption
probability $\alpha_1=\alpha$ and $\alpha_2=1-\alpha$.  For both the
CCE and SE loss functions \eqref{eq:cce_mse_loss}, 
the function $\f^* $ that minimizes the asymptotic empirical risk
$J(\f)$  \eqref{Jf} is 
			\begin{equation}\label{minf:2}
	\f^* ( x ) = \begin{cases}
	\left( 1-\lambda + \lambda \alpha, \lambda (1-\alpha) \right), \quad & \x \in D_1,
	\\
	\left( \lambda \alpha,  1- \lambda \alpha \right), \quad & \x \in  D_2.
	\end{cases}
	\end{equation}
The classification is completely recovered if and only if 
\begin{equation}\label{ReCon2}
1-\frac{ 1}{2 \lambda} < \alpha < \frac{1 }{2 \lambda},
\end{equation} 
which means $\hf^* (\x) = \y( \x)$ for all $\x \in {\mathcal X}$.
\end{corollary}


\begin{corollary}\label{cor:eqA}
Consider classification problem with symmetric corruption probability, i.e.,
	\begin{equation}\label{eqProb}
	\alpha_1=\alpha_2 = \dots= \alpha_n=\frac{1}{n}, \qquad n\geq 2.
	\end{equation}
Then, for both the CCE and SE loss functions \eqref{eq:cce_mse_loss},  
the function $\f^* $ that minimizes the asymptotic empirical risk
$J(\f)$ \eqref{Jf} is
		\begin{equation}\label{minf:nsp}
\f^* ( \x ) = \begin{cases}
\left( 1-\lambda + \frac{\lambda}n , 
\frac{\lambda}n ,
\cdots, 
\frac{\lambda}n
\right), \quad & {\rm if}~ \x \in D_1,
\\
\cdots&
\\
\left(  \frac{\lambda}n, 
\cdots, 
\frac{\lambda}n,
1-\lambda + \frac{\lambda}n
\right), \quad & {\rm if}~ \x \in D_n.
\end{cases}
\end{equation}
If $0\le \lambda < 1$, then $ \hf^* ( \x) = \y (\x)$ for all $ \x \in \mathcal X$, and the classification is completely recovered. 
%If $\lambda = 1$, then 
%$\hf^* ( \x )  = (\frac1n, \frac1n,\dots, \frac1n)$, and 
%the classification cannot be completely. 
\end{corollary}


\subsection{Post-Modified Classifier}
The analysis in the previous section suggests a way to modify the
trained classifier, so that the classification can become completely
recovered, even if label corruptions do not satisfy the condition \eqref{ReCondition}.
We refer this as post-modified classifier, because it can
be applied after the training is completed.

%In the previous analysis, we have shown that the classification is not always completely recovered when the label corruptions do not follow uniform distribution. 
When the corruption probability $\{\alpha_k\}_{1\le k \le n}$ and
proportion $\lambda$ are known, via certain estimation procedure such
as \cite{sukhbaatar2014training,patrini2017making,hendrycks2018using},
we propose to use the following modified classification function:
\begin{equation}\label{fmod}
\f^{mod} (\x) =  \f^* ( \x) + \f_\Delta, 
\end{equation}
where $\f^* $ minimizes the asymptotic empirical risk
$J(\f)$ \eqref{Jf}  and $\f_\Delta$ is constant vector
\begin{equation}
\label{eq:correction}
\f_\Delta := \left( { \lambda \Big(\frac1n - \alpha_1 \Big) } , 
{ \lambda \Big(\frac1n -\alpha_2 \Big) },
\dots, 
{ \lambda \Big(\frac1n -\alpha_n \Big) }
\right).
\end{equation}

As a direct consequence of Theorem \ref{thm:nd}, we have the following conclusion. 


\begin{theorem}\label{thm:mod}
	For both the CCE and SE loss functions \eqref{eq:cce_mse_loss}, the modified classification function defined in \eqref{fmod} satisfies
			\begin{equation}\label{fmod:n}
	\f^{mod} ( \x ) = \begin{cases}
	\left( 1-\lambda + \frac{\lambda}n , 
	\frac{\lambda}n ,
	\cdots, 
	\frac{\lambda}n
	\right), \quad & {\rm if}~ \x \in D_1,
	\\
	\cdots &
	\\
	\left(  \frac{\lambda}n, 
	\cdots, 
	\frac{\lambda}n,
	1-\lambda + \frac{\lambda}n
	\right), \quad & {\rm if}~ \x \in D_n.
	\end{cases}
	\end{equation}
	If $0 \le \lambda < 1$, the classifier $\hf^{mod} ( \x)$ associated with the function $\f^{mod} ( \x )$ satisfies  
	$$ \hf^{mod} ( \x) = \y (\x), \qquad \x \in \mathcal X.$$ 
	%which means the classification is completely recovered. 
\end{theorem}


Theorem \ref{thm:mod} indicates that 
the modified classifier $\hf^{mod} $ can completely recover the exact classification for any $\{\alpha_k\}_{1\le k \le n}$ and any $0\le \lambda< 1$.

\begin{remark}
For symmetric corruption probability
$\alpha_1=\alpha_2=\dots=\alpha_n=\frac1n$, we have $\f_\Delta = {\bf
  0}$.  The modified classification function \eqref{fmod} becomes the
unmodified one.  This is consistent with the result of Corollary \ref{cor:eqA}. 
\end{remark}














==> FirstVersion(arxiv)/Conclusion.tex <==
\section{Conclusion} \label{sec:conclusions}

In this paper, we proposed a correction algorithm for the classification problems, where the data available are potentially corrupted. When the model is trained by minimizing the CCE or SE loss function, given sufficiently large amount of data, it is theoretically shown that the classification can be completely recovered by adding a correction step to the trained model. In particular, if the training data contains unlabeled samples, a random label assignment according to the uniform distribution would make the classification completely recovered. The proposed algorithm is non-intrusive and can be coupled with many models, such as support vector machines, neural networks of various architectures and so on. 
Numerical experiments were conducted with the proposed correction procedure applied to the neural networks models for two academic examples as well as two benchmark real-world tests with complicated and limited dataset. 
Numerical results confirmed
the theoretical findings and demonstrated that, when the data labels contain corruptions, the proposed correction algorithm 
 gives satisfactory test accuracy and can effectively eliminate the impact of label corruptions.

==> FirstVersion(arxiv)/Extension.tex <==
\subsection{Extension} \label{eq:discussion}

Our main theoretical results from Section \ref{sec:analysis} can be
extended to a more general setting, by extending the basic
assumption of the corruption probability \eqref{Yprob} 
More specifically,  we assume that, for each sample $\x_i\in S_c$, its observed label $\ty({\x_i})$ is a realization of a random variable $\mathbf{Y}$ with the distribution 
\begin{equation}\label{Yprob1}
{\rm Prob}(\mathbf{Y}=\ve_j ~|~ \y({\x_i}) = \ve_i )=\alpha_{i,j}, \qquad 1\le i,j \le n.
\end{equation}
This is the probability that the label ${\bf e}_i$ is corrupted to
${\bf e}_j$ and satisfies the obvious condition
$$
\sum_{j=1}^n \alpha_{i,j} = 1, \qquad 1\le i \le n.
$$
Let ${\bf A} :=(\alpha_{i,j})$ be the corruption probability matrix. and we have the following result, as
an extension of Theorem \ref{thm:nd}.
%
\begin{theorem} \label{thm:nd23}
	For both the CCE and SE loss functions
        \eqref{eq:cce_mse_loss}, the function $\f^* $ that minimizes
        the asymptotic empirical risk $J(\f)$  \eqref{Jf} is
	\begin{equation*}
\begin{aligned}
	\f^* ( \x )  &= 
	\begin{cases}
	\left( 1-\lambda + \lambda \alpha_{1,1} , 
	\lambda \alpha_{1,2},
	\dots, 
	\lambda \alpha_{1,n}
	\right), \quad &{\rm if}~\x\in D_1 ,
	\\
	\cdots &
	\\
	\left( \lambda \alpha_{j,1} , \dots
	\lambda \alpha_{j,j-1}, 1-\lambda + \lambda \alpha_{j,j}, \lambda \alpha_{j,j+1}
	\dots, 
	\lambda \alpha_{j,n}
	\right), \quad &{\rm if}~\x\in D_j ,	1<j<n,
	\\
	\cdots &
	\\
	\left(  \lambda \alpha_{n,1} , 
	\lambda \alpha_{n,2},
	\dots, 
	1-\lambda + \lambda \alpha_{n,n} 
	\right), \quad &{\rm if}~\x\in D_n .		
	\end{cases}
	\\[2mm]
	&=
	\left( (1-\lambda) {\bf I} + \lambda {\bf A}^\top \right)  \y (\x), \qquad \forall \x \in \mathcal X.
\end{aligned}
	\end{equation*}
\end{theorem}

\begin{proof}
	The proof is similar to the proof of Theorem \ref{thm:nd} and is omitted.
\end{proof}

Suppose the corruption probability matrix $\bf A$ and corruption
proportion $\lambda$ are known, via statistical estimation procedures
such as those in
\cite{sukhbaatar2014training,patrini2017making,hendrycks2018using},  and matrix $(1-\lambda) {\bf I} + \lambda {\bf A}^\top$ is nonsingular, we propose the following new modified classification function
\begin{equation*}
\f^{mod} (\x) = \left( (1-\lambda) {\bf I} + \lambda {\bf A}^\top \right)^{-1} \f^* (\x).  
\end{equation*}
This modified classification function can completely recover the exact classification for any $\lambda \in [0,1)$ and any transition matrix ${\bf A}$ satisfying $\det( (1-\lambda) {\bf I} + \lambda {\bf A}^\top) \neq 0$.





==> FirstVersion(arxiv)/Introduction.tex <==
\section{Introduction} \label{sec:intro}

Classification problems arise in many practical applications, such as image classification, speech recognition, spam filtering, and so on. Over the past decades, classification has been widely studied by using machine learning techniques, which seek to learn a classifier from labeled training dataset to predict class labels for new data. 
However, real-world datasets often contain noise and their class labels can be corrupted, i.e., mislabelled. This can be caused by a variety of reasons, including human error, measurement error, or subjective bias by labelers, etc.
Label corruptions also occur in data poisoning \cite{li2016data,steinhardt2017certified}. For a more comprehensive review of the sources of label corruptions, see Section B of \cite{frenay2014classification}. 
%On the other hand, in many large scale classification problems, labels in training data may not reliable, because they  
%are often collected through crowd sourcing or by automatically using information on the web  (e.g., web crawling for images \cite{xiao2015learning}) . 
Label corruptions, natural or malicious, can adversely impact classification performance of classifiers. See, for example, \cite{zhang2003robustness, zhu2004class, Nettleton2010} for impacts on
different machine learning techniques. 
It is therefore important to explore robust techniques that can mitigate, or even eliminate, the consequences of label corruptions. 


\subsection{Related work}

There exist a large amount of literature on learning of classifiers in the presence of label noises/errors. See, for example, \cite{frenay2014classification} for 
a detailed survey. 
%Robustness to label corruptions is very important in supervised learning models for classification 
%and has received increasing attention in recent years. 
%
Methods to enhance model robustness against label noises include modifying network architecture and introducing corrections to loss function \cite{larsen1998design, patrini2017making, hendrycks2018using}. Larsen et al.~\cite{larsen1998design} proposed a framework for designing robust neural network classifiers by introducing a probabilistic model
for corruptions. Mnih and Hinton \cite{mnih2012learning} introduced two 
robust loss functions to deal with incomplete or poorly registered labels for binary classification of aerial images. 
In \cite{sukhbaatar2014training}, 
Sukhbaatar et al.~suggested introduction of a
noise layer into neural network models to adapt the network outputs to match the noisy label distribution. The
parameters of the noise layer was estimated as part of the training process and
involved modifications to current training infrastructures for deep network \cite{sukhbaatar2014training}. 
Later, Patrini et al.~\cite{patrini2017making} developed two procedures
for loss function correction, based on transition matrix measuring the probabilities of each class being corrupted into
another. 
They also proposed an estimate of those probabilities \cite{patrini2017making}, by extending the noise estimation technique in \cite{menon2015learning} 
to multi-class setting. 
The readers are also referred to \cite{xiao2015learning,veit2017learning,li2017learning,hendrycks2018using} for more studies on label noise robustness and loss correction techniques under the assumption that one has access to a small subset of clean data during training. 

Efforts were also made to design inherently noise-tolerating (also called noise-robust) algorithms or loss functions. 
For binary classification, it was proved that 0-1 loss is robust to 
symmetric or uniform label noises, while most of the standard convex loss functions are not
\cite{long2010random,manwani2013noise}. 
Several theoretically motivated noise-tolerating 
loss functions, including ramp loss, unhinged loss and savage loss, 
have been introduced in the context of support vector machines (cf.~\cite{brooks2011support,van2015learning,masnadi2009design}).
For binary classification, Natarajan et al.~\cite{natarajan2013learning} proposed an approach to modify any given surrogate loss function to achieve noise robustness.
In the context of deep neural networks, 
Ghosh et al.~\cite{ghosh2015making,ghosh2017robust} derived sufficient conditions for loss function to be robust 
against label corruptions for binary classification \cite{ghosh2015making} and multi-class classification \cite{ghosh2017robust}. 
Recently, Zhang and Sabuncu \cite{zhang2018generalized} 
%observed that the loss based on mean absolute error (MAE), although theoretically robust \cite{ghosh2017robust}, can concurrently cause increased difficulty in training. To combat this drawback, they 
%presented 
generalized the commonly-used categorical 
cross entropy (CCE) loss to 
a set of noise-robust loss functions, which includes mean absolute error (MAE) loss as a special case.  
Other techniques that address various aspects of learning with noisy labels. 
They include, but are not limited to, cleaning up noisy labels \cite{veit2017learning,northcutt2017learning}, directly modelling the label noise and then using the expectation-maximization algorithm to learn the distribution of the true labels \cite{xiao2015learning,khetan2017learning}, and reweighting the samples according to the confidence in them \cite{ liu2016classification, ren2018learning, jiang2017mentornet}.



\subsection{Contributions of the present paper}

The focus of this paper is on a novel correction algorithm for multi-class classification problems with corrupted training data. 
A distinct feature of our algorithm is that the correction procedure is applied to the output of a pre-trained model. That is, it does not require modification to a particular model training method and  is performed only after the completion of the model training.
Therefore, our correction method is \textit{non-intrusive} and highly flexible for practical computations. The non-intrusive feature is not available for many of the aforementioned existing techniques
%represents a significant gain in terms of development cost.
%Such a property is not enjoyed by many existing aforementioned techniques
(cf.~\cite{larsen1998design,mnih2012learning,sukhbaatar2014training,patrini2017making,hendrycks2018using}), most of which require
modification to the model training architecture and/or loss function.
The proposed correction procedure in this paper, on the other hand, can be readily coupled with any existing classification methods, such as logistic regression or deep neural network learning, provided that categorical 
cross entropy (CCE) loss or
squared error (SE) loss is employed. 
The proposed correction algorithm is based upon our theoretical analysis for classification problems with corrupted dataset. 
We prove that, for sufficiently large dataset, the impact of corruption errors is minimal. More precisely, upon applying the proposed correction algorithm, the classification results
become exact, as if there is no data correction, when the size of dataset approaches infinity.
% In another word, the corrected models deliver the correct classification results as if there are no corruptions in the label.
We also derive conditions, under which the original model without using the correction algorithm becomes inherently robust against label corruptions. Moreover, if  
the probability of mis-classification is uniform, we prove that the classification results are always correct in the limit of infinitely large dataset, provided that  a (small) portion of clean data exists in the dataset. 
Numerical examples are provided to confirm the theoretical analysis and 
demonstrate the performance of the proposed correction algorithm. 

This paper is organized as follows. After the basic problem setup in Section \ref{sec:setup}, we present some theoretical analysis on classification problem with corrupted labels in
Section \ref{sec:analysis}. Based on the analysis,
our non-intrusive correction algorithm is then presented in Section \ref{sec:method}. 
Extensions of the analysis and algorithm to more general cases are presented in Section \ref{eq:discussion}.
In Section \ref{sec:examples}, we present an extensive set of numerical examples, including 
well known benchmark problems using real-word datasets, to 
verify the theoretical findings and 
demonstrate the effectiveness of the proposed correction 
algorithms.





==> FirstVersion(arxiv)/Method.tex <==
\section{Implementation and Extension}

\subsection{Implementation Algorithm}\label{sec:method}

In this section, we discuss implementation detail of the aforementioned classification method. Note that the theoretical analysis in the previous section does not depend on the type of
approximation for $\f$ -- it can be linear regression, nonlinear neural networks, etc. Our discussion here is in the context of neural network (NN), because it is the predominant methods used for classification problems, see, for example, \cite{graves2013speech, he2016deep}.
% we will focus ourselves on the neural networks (NN) in both the algorithm description and the numerical examples, since in recent years the NN has achieved great success and popularity in solving the classification problems,
%For a thorough introduction to the NN, one can refer to the review paper \cite{lecun2015deep} and the book \cite{GoodfellowBC-2016}.
%It employs sufficiently large amount of data to train neural networks to learn the classification function $ {\bf f} ({\bf x})$, 
%and then corrects the learned classification function inspired by \eqref{fmod}.  


Assume we are given a sample set $S=\{{\bf x}_i\}_{i=1}^M$, the corresponding observed labels $\{ \ty ({\bf x}_i) \}_{i=1}^M$, 
the corruption ratio $\lambda$ and the corruption distribution $\{ \alpha_j \}_{j=1}^n$. 
As illustrated in Fig.~\ref{fig:algorithm}, the implementation of our algorithm is outlined as follows. 

\begin{description}
	\item[Step 1] Construct a neural network (NN) with $\x$ as  input to approximate the probability function. Let $ {\bf f}: \mathbb R^d \to \mathbb R^n $ be the operator of the NN, where $\Theta$ is the parameter set including all the parameters in the network. 
	 To ensure the output always belongs to the probability simplex $\C$, we exploit the standard softmax function $\sigma ( {\bf z} )$, defined by 
	 $$
	 \sigma ({\bf z})_j =  \frac{ e^{z_j} }{ \sum_{i=1}^n e^{z_i} }, 
	 $$
	  in the output layer of the network. 
	\item[Step 2] Train the network via minimizing the empirical risk \eqref{risk} with either CCE or SE loss function  \eqref{eq:cce_mse_loss}. Let $\Theta^*$ be the trained parameters and $ {\bf f} (\x \Theta^*) $ be the trained network.
	\item[Step 3] Employ the non-intrusive post-correction \eqref{fmod}
          \begin{equation*}
            %\label{post-correct}
	 {\bf f}^{mod} (\x) = {\bf f} (\x; \Theta^*) +  \f_\Delta.
       \end{equation*}
	\item[Step 4] Build the final classifier by argmax procedure:
\begin{equation}\label{DefC}
\hf^{mod} (\x)= \ve_i, \quad  i=\argmax_{j\in \{ 1,2,\ldots,n \} }  f^{mod}_j.
\end{equation}
\end{description}


A graph illustrating the steps is in Figure \ref{fig:algorithm}.
\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.99\textwidth]{AlgorithmFlowchart.pdf}	
	\caption{\small
		Algorithm flowchart.
	}\label{fig:algorithm}
\end{figure}

%\begin{remark}
 Note that Step 3 and Step 4 are applied only after the network training has been completed. Therefore, they are ``non-intrusive'' and do not require modification to the NN structure or training. These steps can be applied to any suitable NN for classification problems.
% \end{remark}


%\begin{remark}
%The trained function $\f (\x; \Theta^*)$ is different from the function $\f^* (\x) $ that minimizes the asymptotic empirical risk $J(\f)$, because of the learning errors as well as the difference between the two functionals $\E(\f)$ and $J(\f)$. However, when $M$ is sufficiently large and the NN model is sufficiently accurate, the two functions $\f (\x; \Theta^*)$ and $\f^* (\x) $ can be very close. 
%\end{remark}
%
%\begin{remark}
%	The correction $\f_\Delta$ in \eqref{eq:correction} depends on the corruption ratio $\lambda$ and the corruption distribution $\{\alpha_k\}_{1\leq k\leq n}$. The estimate of the corruption parameters is another challenging problem and have been investigated by many authors such as \cite{sukhbaatar2014training,patrini2017making,hendrycks2018using}. 
%	Any of these methods could be applied here to give estimates for the corruption rate and distribution. How to design more effective estimate is not the focus of this paper but may be pursued in a separate future study.  
%\end{remark}




















==> FirstVersion(arxiv)/Setup.tex <==
\section{Problem Setup} \label{sec:setup}
Let $D_1, D_2, \ldots, D_n$ be $n$ non-overlapping regions in $\R^d$ with $D_i\cap D_j=\emptyset$ for $i\neq j$.
A feature set is defined to be $\X=\bigcup_{k=1}^n D_k$ and  equipped with a probability measure $\omega$.
%For the sake of simplicity, we assume But our theoretical results and algorithms can be generalized with little effort to the case where $\int_{D_j\cap D_i}\,d\omega=0,\, i\neq j$. 
%
Each feature $\x\in \X$ is associated with a label $\y(\x)$. We use one-hot encoding for the label, i.e., $\y(\x)=\ve_k$ if $\x \in D_k$, where $\ve_{k}\in \R^n$ is $n$-vector with value $1$ in its $k$th component and $0$ otherwise. Let $\Y=\{\ve_k\}_{k=1}^n$ denote the label set. 

We are given a sample set $S=\{\x_i\}_{i=1}^M$, which are i.i.d. drawn from $(\X, \omega)$. For each sample $\x_i$, let $\ty({\x_i})$ be its observed label, which may be corrupted and different from the true label $\y ({\x_i})$.
We assume a subset of the labels $S_c\subset S$ are corrupted and denote its proportion to the entire dataset as $\lambda\in [0, 1)$, i.e., $|S_c|=\lambda M$.
%To be more specific, let $S_c\subset S$ denote the set of samples, of which the labels are untrusted, and we assume $|S_c|=\lambda M$.
For each sample $\x_i\in S_c$, we assume its observed label $\ty({\x_i})$ is a realization of a random variable $\mathbf{Y}$ with distribution 
\begin{equation}\label{Yprob}
{\rm Prob}(\mathbf{Y}=\ve_j)=\alpha_j, \qquad j=1,\dots,n, 
\end{equation}
where $\alpha_j\in [0,1]$ and $\sum_{j=1}^n\alpha_j=1$. We assume that the corruption ratio $\lambda$ and the distribution $\{\alpha_j\}_{j=1}^n$ are available (or can be reliably estimated). However, no prior information is available about the corrupted subset $S_c$. 

Let $\C :=\{\p\in \R^n: p_i\geq 0,\, \sum_{i=1}^n p_i=1\}$ be the probability simplex, where $p_i$ is the probability of a feature to be in $D_i$. We seek to learn  
 a probability function $\f =(f_1,\dots,f_n): \X\rightarrow \C$ and define a classifier
\begin{equation}\label{DefClassifier}
\hf(\x)= \ve_i, \quad  i=\argmax_{j\in \{ 1,2,\ldots,n \} } f_j.
\end{equation}
If maximum probability is attained by multiple labels, we define the first one as the predicted classifier. 
The classification \textit{completely recovered}, if for any $\x\in \X$,  we have $\hf(\x)=\y({\x})$. That is, the classification is able to correctly produce the true classification.

We employ neural networks to train the classifier via minimizing the following empirical risk
\begin{equation}\label{risk}
	\E(\f):=\frac{1}{M}\sum_{i=1}^M L(\ty({\x_i}), \f(\x_i;\Theta)),
\end{equation}
where 
$\Theta$ denotes the model parameters in the network and $L: \Y\times {\mathcal C}\rightarrow \R^+ \cup \{ 0 \}$ is the loss function. We are interested in the commonly used categorical cross-entroy (CCE) and squared-error (SE) loss functions, defined as
\be\label{eq:cce_mse_loss}
L(\p, \q):=
\begin{cases}
	-\sum_{i=1}^n p_i \log q_i, & \text{CCE},\\
	\sum_{i=1}^n |p_i-q_i|^2, & \text{SE}.
\end{cases}
\ee
Let $\Theta^*$ be the network parameters upon satisfactory training and $\f (\x; \Theta^*)$ be the trained model. 

%Since the model is trained using the samples with corrupted labels $\{(\x_i, \ty({\x_i}))\}_{i=1}^M$, in general, we do not expect the classification to be completely recovered. In the following, we show that under certain conditions on the corruption parameters $\lambda$ and $\{\alpha_i\}_{i=1}^n$, the classification can be completely recovered as long as the sample size is sufficiently large. Moreover, if the corruption parameters are known a-priorly or can be estimated from the training data, a correction algorithm will be proposed to render the classification completely recovered.



